Taxonomy of Abstractive Dialogue Summarization: Scenarios, Approaches and Future Directions

Abstractive dialogue summarization is to generate a concise and fluent summary covering the salient information in a dialogue among two or more interlocutors. It has attracted great attention in recent years based on the massive emergence of social communication platforms and an urgent requirement for efficient dialogue information understanding and digestion. Different from news or articles in traditional document summarization, dialogues bring unique characteristics and additional challenges, including different language styles and formats, scattered information, flexible discourse structures and unclear topic boundaries. This survey provides a comprehensive investigation on existing work for abstractive dialogue summarization from scenarios, approaches to evaluations. It categorizes the task into two broad categories according to the type of input dialogues, i.e., open-domain and task-oriented, and presents a taxonomy of existing techniques in three directions, namely, injecting dialogue features, designing auxiliary training tasks and using additional data.A list of datasets under different scenarios and widely-accepted evaluation metrics are summarized for completeness. After that, the trends of scenarios and techniques are summarized, together with deep insights on correlations between extensively exploited features and different scenarios. Based on these analyses, we recommend future directions including more controlled and complicated scenarios, technical innovations and comparisons, publicly available datasets in special domains, etc.

==> datatable.tex <==
\cut{%%%%%
%\begin{sidewaystable}
\begin{table}
\centering
\subtable[Open-domain Dialogue Summarization]{	
\begin{tabular}{|ccccp{3cm}<{\centering}p{2cm}<{\centering}c|}
	%|l|c|c|c|c|c|c|
	\hline
	Name & \makecell{$\#$Samples \\ train/val/test} & $\#$Speakers & Lang. & Desc. & Down. & AVL \\
	\hline
	\multicolumn{7}{|l|}{\bf \em{Dialy Chats}} \\
	\tabincell{c}{SAMSum\cite{gliwa2019samsum}} & 14,732/818/819 & $\geq$2 & Eng. & \tabincell{l}{Dialogues and gold \\ summaries in dataset \\ are human-annotated.}& \tabincell{l}{https://www.\\tensorflow.org/\\datasets/catalog/\\samsum}& Y \\
	\makecell{DialSumm\cite{chen2021dialsumm}} & & & & & & \\
	\makecell{GupShup\cite{mehnaz2021gupshup}} & & & & & & \\
	
	\hline
			
\end{tabular}	
\label{tab:open}		
}
\qquad
\subtable[Task-oriented Dialogue Summarization]{        		
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline
Name & $\#$Samples & $\#$Speakers & Lang. & Desc. & Down. & available \\
\hline
\end{tabular}	
\label{tab:task}
}
\caption{Dialogue Summarization Datasets}	
\end{table}
%\end{sidewaystable}
}%%%%%


\begin{sidewaystable}[thp]
	    \centering
	    \rule{0\textheight}{0.7\textheight}
		\begin{tabular}{|c|c|c|c|l|l|c|}

			\hline
			Name & \makecell{$\#$Samples \\ train/val/test} & $\#$Speakers & Language & Description & Download & AVL \\
			\hline
			\multicolumn{7}{|l|}{\bf \em{Dialy Chats}} \\
			\hline
			\tabincell{c}{SAMSum\cite{gliwa2019samsum}} & 14.7k/0.8k/0.8k%14,732/818/819 
			& $\geq$2 & English & \tabincell{l}{Dialogues and gold summaries in dataset  \\are human-annotated.}&
			 \tabincell{l}{https://huggingface.co/\\datasets/samsum
			 	%https://www.tensorflow.org/\\datasets/catalog/samsum
		 	}& Y \\
			 \hline
			\makecell{DialSumm\cite{chen2021dialsumm}} & 12.5k/0.5k/0.5k%12,460/500/500 
			& 2& English &\tabincell{l}{Dialogue data are collected from public \\dialogue corpora and each dialogue has 3 \\manually annotated reference summaries.} &\tabincell{l}{https://github.com/cylnlp/\\DialogSum} & Y\\
			\hline
			\makecell{GupShup\cite{mehnaz2021gupshup}} & 5.8k/0.5k/0.5k %5,831/500/500
			& $\geq$2 &  \tabincell{l}{Hindi-\\English}& \tabincell{l}{The dialogues and summaries are \\sampled from SAMSum and manually \\translated from English to Hindi-English.}& \tabincell{l}{https://huggingface.co/\\midas/gupshup\_h2e\_mbart} &Y \\
			\hline
			\multicolumn{7}{|l|}{\bf \em{Dramatic Dialogues}} \\
			\hline
			\tabincell{c}{CRD3\cite{rameshkumar2020storytelling}} &
			26.2k/3.5k/4.5k %26,232/3,470/4,541 
			& $>$2 & English & \tabincell{l}{Dialogues and  summaries are collected \\ from {\em Critical Role} episode and Fandom \\ wiki respectively. }&
			\tabincell{l}{https://github.com/\\RevanthRameshkumar/\\CRD3}& Y \\
			\hline
			\tabincell{c}{MediaSumm\\ \cite{zhu2021mediasum}} &
			463.6k/10k/10k %463,6000/10,000/10,000
			& $>$2 & English & \tabincell{l}{Dialogues are interview transcripts and\\ the summaries are the corresponding \\ overview and topic descriptions. }&
			\tabincell{l}{https://github.com/\\zcgzcgzcg1/MediaSum/}& Y \\
			\hline\tabincell{c}{SubTitles\cite{malykh2020sumtitles}} & 153k & $>$2 & English & \tabincell{l}{Dialogues are collected from movies and \\series episodes, and summaries are the \\corresponding captions.}&
			\tabincell{l}{https://github.com/\\huawei-noah/sumtitles}& N \\
			\hline
			\tabincell{c}{SummScreen\\\cite{chen2021summscreen}} &22.6k/2.1k/2.1k %22,588/2,133/2,130
			& $>$2 & English & \tabincell{l}{Dialogues are TV series transcripts and \\summaries are written by human.}&
			\tabincell{l}{https://github.com/\\mingdachen/SummScreen}& Y \\
			\hline
			\multicolumn{7}{|l|}{\bf \em{Debates \& Comments}} \\
			\hline
			\tabincell{c}{ADSC\cite{misra2015using}} & 45%
			& 2 & English & \tabincell{l}{Dialogues are extracted from Internet \\ Argument Corpus. Each dialogue has 5 \\ human-written summaries.}&
			\tabincell{l}{https://nlds.soe.ucsc.edu/\\summarycorpus}& Y \\
			\hline
			\makecell{CQASUMM\cite{chowdhury2019cqasumm}} & 1000k%
			& - & English &\tabincell{l}{Summaries are the best answers and \\ other answers are source documents.} &\tabincell{c}{-} & N\\
			\hline
			\makecell{ConvoSumm\cite{fabbri2021convosumm}} &  -/0.25k/0.25k%
			& $\geq$2 &  \tabincell{l}{English}& \tabincell{l}{ The documents and summaries are from \\comments, discussion and QAs.}& \tabincell{l}{https://github.com/\\Yale-LILY/ConvoSumm} &Y \\
			\hline
		\end{tabular}	
	    \caption{Open-domain Dialogue Summarization}	\label{tab:open}	
\end{sidewaystable}

\begin{sidewaystable}[thp]
	\centering
	\rule{0\textheight}{0.7\textheight}
	\begin{tabular}{|c|c|c|c|l|l|c|}
		
		\hline
		Name & \makecell{$\#$Samples \\ train/val/test} & $\#$Speakers & Language & Description & Download & AVL \\
		\hline
		\multicolumn{7}{|l|}{\bf \em{Customer Service}} \\
		\hline
		\tabincell{c}{\citet{zou2021topic}} & 17.0k/0.9k/0.9k%18.86k 90%/5%/5% 
		& 2 & Chinese & \tabincell{l}{Dialogues are between a customer and a \\ service agent. Summaries are brief \\descriptions written by agents.
		}&
		\tabincell{l}{https://github.com/Rowit\\Zou/topic-dialog-summ
		}& Y \\
		\hline
		\makecell{\citet{lin2021csds}} & 9.1k/0.8k/0.8k%9,101 / 800 / 800
		& 2& Chinese &\tabincell{l}{Dialogues are between users and agents. \\Each dialogue has an overall summary, \\user summary and agent summary.} &\tabincell{l}{https://github.com/\\xiaolinAndy/CSDS} & Y\\
		\hline
		\makecell{\citet{zou2021unsupervised}} & -/0.5k/0.5k%1.09M chat logs
		& 2 &  \tabincell{l}{Chinese}& \tabincell{l}{No (dialogue, summary) training pairs. \\ The gold summaries in val and test sets \\are written by human.}& \tabincell{l}{https://github.com/Rowit\\Zou/RankAE} &Y \\
		\hline
		\tabincell{c}{Didi\cite{liu2019automatic}} &
		296.3k/2.9k/29.6k %26,232/3,470/4,541 
		& 2 & Chinese & \tabincell{l}{The dialogues are between users and \\agents, and the summaries are written \\ by agents.}&
		\tabincell{l}{-}& N \\
		\hline
		\tabincell{c}{TWEETSUMM\\ \cite{feigenblat-etal-2021-tweetsumm-dialog}} &
		0.9k/0.1k/0.1k %1.1k 80%/10%/10%
		& 2 & English & \tabincell{l}{Dialogues are from Tweets. Summaries \\ are generated by human annotators.}&
		\tabincell{l}{https://github.com/guyfe/\\Tweetsumm}& Y \\
		\hline\tabincell{c}{TODSum\cite{zhao2021todsum}} & 9.9k & 2 & English & \tabincell{l}{Dialogues are from MultiWOZ\cite{eric2019multiwoz}. \\ Summaries are generated by \\ Template2Text model SC-GPT\cite{peng2020few} \\with human evaluation and correct.}&
		\tabincell{l}{-}& N \\
		\hline
		\multicolumn{7}{|l|}{\bf \em{Court}} \\
		\hline
		\tabincell{c}{Justice\cite{fuzw20}} & 30k%14,732/818/819 
		& 2 & Chinese & \tabincell{l}{The court debate transcript is the input \\and the fact description is summary.}&
		\tabincell{l}{-}& N \\
		\hline
		\makecell{PLD\cite{duan2019legal}} & 5.5k%
		& $\geq$2 & English &\tabincell{l}{Dialogues are court records. Summaries \\are pre-generated by the case judge.
		} &\tabincell{l}{https://github.com/zhou\\xinhit/Legal\_Dialogue\\ \_Summarization} & Y\\
		\hline
		\makecell{\citet{xi2020global}} &  30.8/3.8k/3.8k%38.5k 80%/10%/10%
		& 2 &  Chinese& \tabincell{l}{ Dialogues are police inquiry records.\\ Summaries are manually tagged.}& \tabincell{l}{http://eie.usts.edu.cn/prj/\\NLPoSUST/LcsPIRT.htm} &Y \\
		\hline
	\end{tabular}	
	\caption{Task-oriented Dialogue Summarization (1)}	\label{tab:open}	
\end{sidewaystable}

\begin{sidewaystable}[thp]
	\centering
	\rule{0\textheight}{0.7\textheight}
	\begin{tabular}{|c|c|c|c|l|l|c|}
		
		\hline
		Name & \makecell{$\#$Samples \\ train/val/test} & $\#$Speakers & Language & Description & Download & AVL \\
		\hline
		\multicolumn{7}{|l|}{\bf \em{Medical Care}} \\
		\hline
		\tabincell{c}{\citet{joshi2020dr}} & 1.4k/0.16k/0.17k%1365 /158/167 
		& 2 & English & \tabincell{l}{Dialogues are from a telemedicine \\ platform. Summaries are written by \\medical doctors.
		}&
		\tabincell{l}{-}& N \\
		\hline
		\makecell{\citet{song2020summarizing}} & 36k/-/9k %35987/8996
		& 2& Chinese &\tabincell{l}{Dialogues are between users and agents. \\Each dialogue has an overall summary, \\user summary and agent summary.} &\tabincell{l}{https://github.com/\\cuhksz-nlp/HET-MC} & Y\\
		\hline
		\makecell{\citet{liu2019topic}} & 100k/1k/0.49k
		& 2 &  \tabincell{l}{English}& \tabincell{l}{Dialogues are between nurses and \\ patients. Summaries are concise \\ descriptions of different attributes of a \\specified symptom. }& \tabincell{l}{-} &N \\
		\hline
		\tabincell{c}{\citet{zhang2021leveraging}} &
		0.9k/0.2k/0.2k %939(15043), 201(3095), and 202(3450),
		& 2 & English & \tabincell{l}{Dialogues and summaries are collected \\ from a simulated Electronic Health \\ Record system.}&
		\tabincell{l}{-}& N \\
		\hline
		\multicolumn{7}{|l|}{\bf \em{Official Affairs (Meeting \& Emails)}} \\
		\hline
		\tabincell{c}{AMI\cite{carletta2005ami}} &
		137 %142 
		& $>$2 & English & \tabincell{l}{Dialogues are transfered from 100 hours\\ of meeting recordings. Summaries are \\manually annotated.}&
		\tabincell{l}{https://groups.inf.ed.\\ac.uk/ami}& Y \\
		\hline\tabincell{c}{ICSI\cite{janin2003icsi}} & 59 %75 
		& $>$2 & English & \tabincell{l}{Dialogues are from natural meetings. \\ Summaries are annotated by human.}&
		\tabincell{l}{https://groups.inf.ed.\\ac.uk/ami/icsi}& Y \\
		\hline
		\tabincell{c}{QMSum\cite{zhong2021qmsum}} & 1.3k/2.7k/2.7k% 1,257 / 272 / 279 
		& $>$2 & English & \tabincell{l}{QMSum contains Product, Academic\\ and Committee meetings.}&
		\tabincell{l}{https://github.com/\\Yale-LILY/QMSum}& Y \\
		\hline
		\makecell{\citet{ulrich2008publicly}} & 30%1800/249/500
		& $>$2 & English &\tabincell{l}{
		} &\tabincell{l}{} & Y\\
		\hline
		\makecell{EmailSum\cite{zhang2021emailsum}} & 1.8k/0.25k/0.5k%1800/249/500
		& $>$2 & English &\tabincell{l}{Dialogues are Email threads. Summaries \\are written by human.
		} &\tabincell{l}{https://github.com/\\ZhangShiyue/EmailSum} & Y\\
		\hline
		\makecell{ConvoSumm\cite{fabbri2021convosumm}} &  -/0.25k/0.25k%
		& $\geq$2 &  \tabincell{l}{English}& \tabincell{l}{Part of documents and summaries in \\ ConvoSumm are from emails.}& \tabincell{l}{https://github.com/\\Yale-LILY/ConvoSumm} &Y \\
		\hline
	\end{tabular}	
	\caption{Task-oriented Dialogue Summarization (2)}	\label{tab:open}	
\end{sidewaystable}
